CoopReflect: Towards Natural Language Communication for Cooperative Autonomous Driving via Multi-Agent Learning

Past work has demonstrated that autonomous vehicles can drive more safely if they communicate with each other. However, this communication is usually not human-understandable. Using natural language as a vehicle-to-vehicle (V2V) communication protocol offers the potential for autonomous vehicles to drive cooperatively not only with each other but also with human drivers. To explore the potential use of natural language for V2V communication, we develop LLM-based driving agents and study their interactions in a new simulation environment, TalkingVehiclesGym, which features traffic scenarios where communication can potentially help avoid imminent collisions and/or support efficient traffic flow. While LLM agents relying solely on chain-of-thought reasoning struggle to coordinate effectively, we introduce CoopReflect, a multi-agent learning framework that equips agents with knowledge for both natural language message generation and high-level decision-making through trial and error and multi-agent debriefing. Experiments show that CoopReflect produces more meaningful and human-understandable messages than existing baselines, enabling stronger cooperation. Finally, we distill scenario-specific knowledge into a unified language model policy, achieving cross-scenario generalization and substantially reducing decision-making latency. Our code and demo videos are available at https://talking-vehicles.github.io/.

==> Tables/experiment_additional.tex <==
\begin{table}[h!]
    \centering
    \caption{\small Experiment Results for Silent,  Zero-shot Comm and Debrief Comm Agents. We evaluate on adversarial cases where being aggressive or conservative will result in failure.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcc|ccc|ccc|ccc}
    \toprule
    \multicolumn{3}{c|}{\diagbox{Method}{Scenario}} & \multicolumn{3}{c|}{Overtake (Perception)} & \multicolumn{3}{c|}{Red Light} & \multicolumn{3}{c}{Left Turn} \\
    \midrule
    Name & LLM & Comm & 
    R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$ & 
    R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$ & 
    R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$\\
    \midrule
     Zero-shot (Silent) & Yes & No & -1.00 & 1.00 & 0.0 & -0.40 & 0.70 & 30.0 & 0.06 & 0.43 & 53.3 \\
     Zero-shot (Comm) & Yes & Yes & -0.76 & 0.76 & 23.3 & 0.60 & 0.07 & 66.7 & 0.46 & 0.10 & 53.3 \\
    Debrief (Comm) & Yes & Yes & 0.43 & 0.26 & 70.0 & 0.76 & 0.00 & 76.7 & 0.86 & 0.03 & 90.0\\
    \midrule
    \multicolumn{3}{c|}{\diagbox{Method}{Scenario}} & \multicolumn{3}{c|}{Overtake (Negotiation)} & \multicolumn{3}{c|}{Highway Exit} & \multicolumn{3}{c}{Highway Merge} \\
    \midrule
     Zero-shot (Silent) & Yes & No & -1.86 & 1.93 & 3.3 & -1.73 & 1.86 & 6.7 & -2.00 & 2.00 & 0.0 \\
     Zero-shot (Comm) & Yes & Yes & 0.40 & 0.80 & 60.0 & -1.43 & 1.70 & 15.0 & -0.40 & 1.2 & 45.5 \\
    Debrief (Comm) & Yes & Yes & 0.73 & 0.50 & 51.6 & -0.16 & 0.93 & 38.3 & 0.96 & 0.50 & 73.3\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:additional}
    \vspace{-6pt}
\end{table} 

==> Tables/experiment_cooperative_perception.tex <==
\begin{table*}[h!]
    \centering
    \caption{\small {\textcolor{brickred}{\texttt{Cooperative Perception}}} Scenarios. \texttt{mean $\pm$ std} over 3 trials, each using 30 evaluation episodes.}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcc|cc|cc|cc}
    \toprule
    \multicolumn{3}{c|}{\diagbox{Method}{Scenario}} &
    \multicolumn{2}{c|}{Overtake (Perception)} &
    \multicolumn{2}{c|}{Red Light} &
    \multicolumn{2}{c}{Left Turn} \\
    \midrule
    Name & LLM & Comm & 
    CR (\%) $\downarrow$ & SR (\%) $\uparrow$ & 
    CR (\%) $\downarrow$ & SR (\%) $\uparrow$ & 
    CR (\%) $\downarrow$ & SR (\%) $\uparrow$\\
    \midrule
    Zero-shot & Yes & No &
        93.3 $\pm$ 3.4 & 0.0 $\pm$ 0.0 &                            %overtake
        93.3 $\pm$ 6.7 & 6.7 $\pm$ 6.7 &                            %red-light
        93.3 $\pm$ 5.8 & 6.7 $\pm$ 5.8 \\                           %left-turn
    +Reflection & Yes & No &
        87.8 $\pm$ 3.4 & 0.0 $\pm$ 0.0 &                           %overtake
        94.4 $\pm$ 6.9 & 5.6 $\pm$ 6.9 &                            %red-light
        76.7 $\pm$ 20.8 & 23.3 $\pm$ 20.8 \\                          %left-turn
    +Correction+RAG & Yes & No &
        62.0 $\pm$ 31.9 & 4.4 $\pm$ 7.7 &                            %overtake
        93.3 $\pm$ 3.3 & 6.7 $\pm$ 3.3 &                           %red-light
        64.4 $\pm$ 15.0 & 35.6 $\pm$ 15.0 \\%left-turn
    \midrule
    Zero-shot & Yes & Yes &
        91.1 $\pm$ 5.1 & 4.4 $\pm$ 5.1 &                           %overtake
        60.0 $\pm$ 11.5 & 38.9 $\pm$ 10.7 &                           %red-light
        85.6 $\pm$ 8.4 & 14.4 $\pm$ 8.4 \\                          %left-turn
    +Reflection & Yes & Yes &
        63.3 $\pm$ 14.5 & 34.4 $\pm$ 10.7 &                            %overtake
        37.8 $\pm$ 18.4 & 47.8 $\pm$ 18.4 &                            %red-light
        51.1 $\pm$ 37.2 & 47.8 $\pm$ 36.0 \\%left-turn
    +Correction+RAG & Yes & Yes &
        4.4 $\pm$ 1.9 & 90.0 $\pm$ 6.7 &           %overtake
        13.3 $\pm$ 12.0 & 66.7 $\pm$ 27.3 &                            %red-light
        43.3 $\pm$ 38.4 & 38.9 $\pm$ 22.7 \\                          %left-turn
    +Debrief & Yes & Yes &
        \textbf{1.1 $\pm$ 1.9} & \textbf{94.4 $\pm$ 6.9} &                   %overtake
        \textbf{0.0 $\pm$ 0.0} & \textbf{93.3 $\pm$ 5.8} & %red-light
        \textbf{6.7 $\pm$ 3.3} & \textbf{92.2 $\pm$ 3.8} \\%left-turn
    \midrule
    \textcolor{gray}{Coopernaut} & \textcolor{gray}{No} & \textcolor{gray}{Yes} &
        \textcolor{gray}{4.5 $\pm$ 3.1} & \textcolor{gray}{90.5 $\pm$ 1.2} & 
        \textcolor{gray}{17.7 $\pm$ 7.8} & \textcolor{gray}{80.7 $\pm$ 7.6} & 
        \textcolor{gray}{18.1 $\pm$ 6.2} & \textcolor{gray}{80.7 $\pm$ 5.2} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:experiment_cooperative_perception}
\end{table*} 

% \begin{table}[h!]
%     \centering
%     \caption{\small Experiment Results for {\textcolor{brickred}{\texttt{Cooperative Perception}}} Scenarios.}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lcc|ccc|ccc|ccc}
%     \toprule
%     \multicolumn{3}{c|}{\diagbox{Method}{Scenario}} &
%     \multicolumn{3}{c|}{Overtake (Perception)} &
%     \multicolumn{3}{c|}{Red Light} &
%     \multicolumn{3}{c}{Left Turn} \\
%     \midrule
%     Name & LLM & Comm & 
%     R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$ & 
%     R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$ & 
%     R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$\\
%     \midrule
%     Zero-shot (Silent) & Yes & No &
%         -0.93  & 93.3  & 0.0  &                            %overtake
%         -0.87  & 93.3  & 6.7 &                            %red-light
%         -0.87  & 93.3  & 6.7  \\                           %left-turn
%     +Reflection (Silent) & Yes & No &
%         -0.26 & 36.7 & 10.0 &                           %overtake
%         -0.87 & 93.3 & 6.7 &                            %red-light
%         -0.27 & 63.3 & 36.7 \\                          %left-turn
%     +Correction+RAG (Silent) & Yes & No &
%         0.07 & 33.3 & 40.0 &                            %overtake
%         -0.73 & 86.7 & 13.3 &                           %red-light
%         0.20 & 40.0 & 60.0 \\%left-turn
%     \midrule
%     Zero-shot (Comm) & Yes & Yes &
%         -0.46 & 73.3 & 26.7 &                           %overtake
%         -0.33 & 66.7 & 33.3 &                           %red-light
%         -1.00 & 100.0 & 0.0 \\                          %left-turn
%     +Reflection (Comm) & Yes & Yes &
%         0.40 & 30.0 & 70.0 &                            %overtake
%         0.07 & 10.0 & 26.7 &                            %red-light
%         \textbf{0.60} & \textbf{20.0} & \textbf{80.0} \\%left-turn
%     +Correction+RAG (Comm) & Yes & Yes &
%         \textbf{0.70} & \textbf{6.7} & 76.7 &           %overtake
%         0.73 & 13.3 & 87.7 &                            %red-light
%         -0.60 & 76.7 & 16.7 \\                          %left-turn
%     +Debrief (Comm) & Yes & Yes &
%         0.63 & 16.7 & \textbf{80.0} &                   %overtake
%         \textbf{1.00} & \textbf{0.0} & \textbf{100.0} & %red-light
%         \textbf{0.60} & \textbf{20.0} & \textbf{80.0} \\%left-turn
%     \midrule
%     \textcolor{gray}{Coopernaut (Comm)} & \textcolor{gray}{No} & \textcolor{gray}{Yes} &
%         \textcolor{gray}{1.00} & \textcolor{gray}{0.0} & \textcolor{gray}{100.0} & 
%         \textcolor{gray}{0.97} & \textcolor{gray}{0.0} & \textcolor{gray}{96.7} & 
%         \textcolor{gray}{1.00} & \textcolor{gray}{0.0} & \textcolor{gray}{100.0} \\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:experiment_cooperative_perception}
% \end{table} 

==> Tables/experiment_negotiation.tex <==
\begin{table*}[h]
    \centering
    \caption{\small {\textcolor{brickred}
    {\texttt{Negotiation}}} Scenarios. \texttt{mean $\pm$ std} over 3 trials, each using 30 evaluation episodes.}
    \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{lcc|cc|cc|cc}
    \toprule
    \multicolumn{3}{c|}{\diagbox{Method}{Scenario}} &
    \multicolumn{2}{c|}{Overtake (Negotiation)} &
    \multicolumn{2}{c|}{Highway Merge} &
    \multicolumn{2}{c}{Highway Exit} \\
    \midrule
    Name & LLM & Comm & 
    CR (\%) $\downarrow$ & SR (\%) $\uparrow$ & 
    CR (\%) $\downarrow$ & SR (\%) $\uparrow$ & 
    CR (\%) $\downarrow$ & SR (\%) $\uparrow$\\
    \midrule
    Zero-shot & Yes & No &
        89.9 $\pm$ 2.8 & 7.2 $\pm$ 3.8 &     % overtake
        100.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 &    % highway-merge
        33.3 $\pm$ 9.3 & 66.1 $\pm$ 9.2\\    % highway-exit
    +Reflection & Yes & No &
        32.8 $\pm$ 29.4 & 36.7 $\pm$ 52.1 &  % overtake
        15.0 $\pm$ 23.1 & 84.4 $\pm$ 22.6 &  % highway-merge
        32.8 $\pm$ 13.4 & 67.2 $\pm$ 13.4 \\ % highway-exit
    +Correction+RAG & Yes & No &
        46.7 $\pm$ 21.9 & 33.3 $\pm$ 28.0 &  % overtake
        35.6 $\pm$ 29.4 & 64.4 $\pm$ 29.4 &  % highway-merge
        33.9 $\pm$ 28.4 & 51.1 $\pm$ 14.2 \\ % highway-exit
    \midrule
    Zero-shot & Yes & Yes &
        87.8 $\pm$ 5.9 & 11.7 $\pm$ 6.7 &   % overtake
        67.2 $\pm$ 27.1 & 32.8 $\pm$ 27.1 & % highway-merge
        53.3 $\pm$ 11.5 & 46.7 $\pm$ 11.5 \\% highway-exit
    +Reflection & Yes & Yes &
        55.6 $\pm$ 38.9 & 43.3 $\pm$ 37.1 & % overtake
        20.0 $\pm$ 1.7 & 80.0 $\pm$ 1.7 &   % highway-merge
        53.9 $\pm$ 24.1 & 45.6 $\pm$ 23.6 \\% highway-exit
    +Correction+RAG & Yes & Yes &
        38.3 $\pm$ 6.0 & 61.1 $\pm$ 5.4 &   % overtake
        40.0 $\pm$ 18.0 & 60.0 $\pm$ 18.0 & % highway-merge
        49.4 $\pm$ 49.2 & 43.3 $\pm$ 39.8 \\% highway-exit
    +Debrief & Yes & Yes &
        \textbf{3.3 $\pm$ 3.3} & \textbf{95.6 $\pm$ 3.8} & %overtake
        \textbf{6.7 $\pm$ 11.5} & \textbf{93.3 $\pm$ 11.5} & %highway-merge
        \textbf{18.3 $\pm$ 21.7} & \textbf{81.1 $\pm$ 21.2} \\ %highway-exit
    \bottomrule
    \end{tabular}
    }
    \label{tab:experiment_negotiation}
\end{table*} 

==> Tables/experiment_zero_shot.tex <==
\begin{table}[h!]
    \centering
    \caption{\small Experiment Results for Communication vs Silent Agents. We evaluate on adversarial cases where being aggressive or conservative will result in failure.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcc|ccc|ccc|ccc}
    \toprule
    \multicolumn{3}{c|}{\diagbox{Method}{Scenario}} & \multicolumn{3}{c|}{Overtake (Perception)} & \multicolumn{3}{c|}{Red Light} & \multicolumn{3}{c}{Left Turn} \\
    \midrule
    Name & LLM & Comm & 
    R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$ & 
    R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$ & 
    R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$\\
    \midrule
    Zero-shot (Silent) & Yes & No & 0.00 & 0.00 & 0.0 & -0.60 & 0.80 & 20.0 & 0.20 & 0.33 & 53.3 \\
    Zero-shot (Comm) & Yes & Yes & -0.63 & 0.66 & 33.3 & 0.80 & 0.07 & 86.7 & 0.20 & 0.33 & 56.7 \\
    Coopernaut & No & Yes & \textcolor{gray}{1.00} & \textcolor{gray}{0.00} & \textcolor{gray}{100.0} & \textcolor{gray}{0.97} & \textcolor{gray}{0.00} & \textcolor{gray}{96.7} & \textcolor{gray}{0.93} & \textcolor{gray}{0.03} & \textcolor{gray}{96.7} \\
    \midrule
    \multicolumn{3}{c|}{\diagbox{Method}{Scenario}} & \multicolumn{3}{c|}{Overtake (Negotiation)} & \multicolumn{3}{c|}{Highway Exit} & \multicolumn{3}{c}{Highway Merge} \\
    \midrule
    Zero-shot (Silent) & Yes & No & 0.50 & 0.67 & 3.3 & -0.93 & 1.5 & 20.0 & -1.26 & 1.63 & 18.5 \\
    Zero-shot (Comm) & Yes & Yes & 0.50 & 0.70 & 53.3 & -0.73 & 0.6 & 33.3 & -0.10 & 1.03 & 45.5 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:comm_ncomm}
    \vspace{-6pt}
\end{table} 

\begin{table*}[h]
    \centering
    \caption{\small {\textcolor{brickred}
    {\texttt{Negotiation}}} Scenarios. \texttt{mean $\pm$ std} over 3 trials, each using 30 evaluation episodes.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcc|cc|cc|cc}
    \toprule
    \multicolumn{3}{c|}{\diagbox{Method}{Scenario}} &
    \multicolumn{2}{c|}{Overtake (Negotiation)} &
    \multicolumn{2}{c|}{Highway Merge} &
    \multicolumn{2}{c}{Highway Exit} \\
    \midrule
    Name & LLM & Comm & 
    CR (\%) $\downarrow$ & SR (\%) $\uparrow$ & 
    CR (\%) $\downarrow$ & SR (\%) $\uparrow$ & 
    CR (\%) $\downarrow$ & SR (\%) $\uparrow$\\
    \midrule
    Zero-shot & Yes & No &
        89.9 $\pm$ 2.8 & 7.2 $\pm$ 3.8 &     % overtake
        100.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 &    % highway-merge
        33.3 $\pm$ 9.3 & 66.1 $\pm$ 9.2\\    % highway-exit
    +Reflection & Yes & No &
        32.8 $\pm$ 29.4 & 36.7 $\pm$ 52.1 &  % overtake
        15.0 $\pm$ 23.1 & 84.4 $\pm$ 22.6 &  % highway-merge
        32.8 $\pm$ 13.4 & 67.2 $\pm$ 13.4 \\ % highway-exit
    +Correction+RAG & Yes & No &
        46.7 $\pm$ 21.9 & 33.3 $\pm$ 28.0 &  % overtake
        35.6 $\pm$ 29.4 & 64.4 $\pm$ 29.4 &  % highway-merge
        33.9 $\pm$ 28.4 & 51.1 $\pm$ 14.2 \\ % highway-exit
    \midrule
    Zero-shot & Yes & Yes &
        87.8 $\pm$ 5.9 & 11.7 $\pm$ 6.7 &   % overtake
        67.2 $\pm$ 27.1 & 32.8 $\pm$ 27.1 & % highway-merge
        53.3 $\pm$ 11.5 & 46.7 $\pm$ 11.5 \\% highway-exit
    +Reflection & Yes & Yes &
        55.6 $\pm$ 38.9 & 43.3 $\pm$ 37.1 & % overtake
        20.0 $\pm$ 1.7 & 80.0 $\pm$ 1.7 &   % highway-merge
        53.9 $\pm$ 24.1 & 45.6 $\pm$ 23.6 \\% highway-exit
    +Correction+RAG & Yes & Yes &
        38.3 $\pm$ 6.0 & 61.1 $\pm$ 5.4 &   % overtake
        40.0 $\pm$ 18.0 & 60.0 $\pm$ 18.0 & % highway-merge
        49.4 $\pm$ 49.2 & 43.3 $\pm$ 39.8 \\% highway-exit
    +Debrief & Yes & Yes &
        \textbf{3.3 $\pm$ 3.3} & \textbf{95.6 $\pm$ 3.8} & %overtake
        \textbf{6.7 $\pm$ 11.5} & \textbf{93.3 $\pm$ 11.5} & %highway-merge
        \textbf{18.3 $\pm$ 21.7} & \textbf{81.1 $\pm$ 21.2} \\ %highway-exit
    \bottomrule
    \vspace{-36pt}
    \end{tabular}
    }
    \label{tab:experiment_negotiation}
\end{table*} 

==> Tables/experiment_zeroshot_train.tex <==
\begin{table}[h!]
    \vspace{-6pt}
    \centering
    \caption{\small Experiment Results for Improvement Methods.}
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{lcc|ccc|ccc}
    \toprule
    \multicolumn{3}{c|}{\diagbox{Method}{Scenario}} &  \multicolumn{3}{c|}{Red Light} & \multicolumn{3}{c}{Highway Merge} \\
    \midrule
    Name & LLM & Comm &
    R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$ & 
    R $\uparrow$ & CR $\downarrow$ & SR $\uparrow$\\
    \midrule
    Zero-shot & Yes & No & -0.6 & 0.80 & 20.0 & -1.26 & 1.63 & 18.5 \\
    +Reflection & Yes & No & -0.73 & 0.86 & 13.3 & -0.86 & 1.43 & 28.5 \\
    +Correction+RAG & Yes & No & -1.00 & 1.00 & 0.00 & -2.00 & 2.00 & 0.0 \\
    \midrule
    Zero-shot & Yes & Yes & 0.80 & 0.07 & 86.7 & -0.10 & 1.03 & 45.5 \\
    +Reflection & Yes & Yes & 0.70 & 0.13 & 83.3 & 0.20 & 0.87 & 50.0 \\
    +Correction+RAG & Yes & Yes & -0.93 & 0.96 & 3.3 & -2.00 & 2.00 & 0.0 \\
    +Debrief & Yes & Yes & 0.80 & 0.07 & \textbf{90.0}& \textbf{0.40} & \textbf{0.57} & \textbf{51.5}\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:zeroshot_train}
\end{table} 

==> contents/1_introduction_old.tex <==
\section{Outline of the Introduction}

1. Importance of multi-agent / V2V communication for collaboration (in the autonomous driving domain).

2. Why use natural language as a medium? (1) It potentially enables human participation (2) Allows proactive strategies for autonomous vehicles when interacting with other vehicles. We can give an example here.

3. Insufficiency in the previous work. (1) For V2V works, they don't consider human interaction and develop reactive policies for autonomous vehicles (2) For LLM for driving work, they don't consider multi-agent interactions. (3) For multi-agent interaction work with natural language, they are not in the driving domain, and the task horizon is usually short, and messages are very simplified.

4. Overview of what we do in this paper.

5. Mention that it is an exploratory work and limitations exist, but it opens up many new research directions.


(By Peter on 12/07)

Notes for intro:

- Driving is inherently multiagent - when humans drive, each person
    makes their own decisions based on their own perceptions.

- As we move towards (semi-)autonomous cars, it may be more efficient to
    centrally control all cars, but that's hugely impractical and would
    never be accepted
- nevertheless there are undeniable advantages to cars working
    cooperatively in a limited capacity

- past work has shown the benefits of cooperative perception by
    (semi-)autonomous cars (Coopernaut)
- however the benefits are limited to the autonomous cars in the
    vicinity
- in a mixed autonom=y setting, human drivers are still left to make
    their decisions solely based on local perceptions.

- We are motivated by the eventual possibility that human drivers - or
    part-time controllers of semi-autonomous cars could enjoy some of
    these cooperative perception benefits.
- To this end, we develop the first cooperative perception system based
    on natural language.

- While this work doesn't go as far as making the system fully human
    usable - that next step, and the requisite associate user studies
     is left for future work - this paper takes an important step in
     that direction.
- Namely, it achieves the benefits of Coopernaut (or starts moving in the direction of acheiving those benefits...), with all the
     communication being done in language

- Steps remaining require making it all real time, and making the
     messages short and understandable.  And making sure they're not too
     distracting to a driver (because their spoken) or a semi-autonomous
     controller (because they're short)

\section{Introduction}

State-of-the-art autonomous driving policies are commonly designed from the perspective of a single agent's sensors. Therefore, to enhance safety, it is essential to account for multi-agent interactions. Among the strategies employed is incorporating motion prediction or intention inference of other traffic participants in decision-making. Some models independently forecast the future movements of these traffic participants \citep{iplan2023}, whereas others account for mutual interactions among autonomous vehicles and other traffic agents \citep{seff2023motionlm}. %\commenta{account for the mutual interaction between the autonomous vehicle (ego vehicle) and other traffic agents} jointly assess how the autonomous vehicle (ego vehicle) might influence them and vice versa \citep{seff2023motionlm}. 
However, the challenge lies in the substantial uncertainty in predicting other drivers' intentions, often resulting in excessively cautious driving strategies \citep{rhinehart2021uncertainty}.

%Given the cooperative nature of the safe driving problem, why not enable vehicles to communicate their intentions and observations directly with each other? \commenta{Given its cooperative nature, the safe driving problem could be largely simplified by enabling vehicles to communicate their intentions and observations with each other.} 
Given its cooperative nature, the safe driving problem could be largely simplified by enabling vehicles to communicate their intentions and observations with each other. The concepts of vehicle-to-vehicle (V2V) and vehicle-to-infrastructure (V2I) communication have recently emerged as a promising approach for multi-vehicle cooperation, garnering considerable research interest~\citep{wang2020v2vnet, cui2022coopernaut,  xu2022v2x, xu2022opv2v}. While the focus of V2V communication has predominantly been on cooperative perception rather than cooperative control, it often employs modalities (latent representations, LiDAR points, locations of objects, etc.,) that are not intuitively nor easily understood by humans, thus requiring that all the participating vehicles be autonomous and share the same protocol. Natural language, as a refined and highly adaptable form of human communication, offers the potential for human drivers to also participate in this cooperation. If vehicles could ``speak" in human language, it would pave the way for developing technologies that facilitate communication between autonomous vehicles and human drivers, enhancing cooperation and understanding in mixed-autonomy traffic environments. Even in fully autonomous settings, a natural language interface could offer flexibility for agents to explain their decisions, talk to other autonomous vehicles with proper translation, quickly adapt to different traffic regulations, and negotiate plans.

% \commenta{I think we should introduce here that LLM-based V2V is not only beneficial in mixed-traffic scenarios - especially since we may not even include human interaction in this first paper -, but also highlight its benefits in terms of using natural language as an interface between autonomous agents - e.g. generalization, coverage, expressiveness, explainability, intuitive integration with rule-based planners,... -. I think if we could come up with a concrete example / scenario in which this approach is superior to traditional traditional V2V protocols it would greatly strengthen the work's motivation. Thoughts?}.



As a concrete example of the power of using language in V2V communication, consider the following scenario, as illustrated in Figure~\ref{fig:intro}. 
A truck has broken down and stopped on a two-way road divided by a yellow dashed line. The vehicles trailing the truck cannot see whether the lane going in the opposite direction is free from oncoming cars, which could allow them to use that lane to safely move around the truck to circumvent the growing traffic jam. If the truck is capable of communication, it could relay a message such as, ``The opposite lane is clear, you may safely perform a lane change to pass me." Alternatively, in busier times, the queued vehicles could initiate a dialogue with oncoming traffic, proposing, ``Can we take turns using the lane to avoid major congestion?" Through simple but effective communication about their intentions or observations, a mixture of human-driven and autonomous vehicles could significantly enhance traffic flow and overall efficiency.

In this work, we first introduce the problem of \task. In this problem setting, a scenario in autonomous driving is formulated as a multi-agent partially observable and general-sum game wherein each traffic participant is pursuing a cooperative goal modulated by individual preferences\footnote{{Generally}, we assume all cars seek a smooth traffic flow. Meanwhile, each car prefers to reach its destination as quickly as possible. {But their goals may conflict with each other's.}}. When conflicts arise or unexpected events occur, vehicles have the opportunity to generate and broadcast messages that contain observations of abnormal events or negotiations to cooperatively reach their goals. The vehicles can then make decisions according to the received messages. 
\input{figure_tex/intro}
Enabling vehicles to \textbf{``talk"} {to each other} with intentions and conveying helpful information {in natural language} presents significant challenges. There are studies like Dolphins \citep{ma2023dolphins} and LINGO-1 \citep{wayve2023lingo1} that have trained Visual-Language-Action models to both make driving decisions and articulate their reasoning to humans. However, training such models requires extensive data. At the time of writing this paper, only a limited number of datasets exist that provide language commentary data for single-agent driving scenarios \citep{kim2018bddx, kim2019HAD, qian2023nuscenesqa, sima2023drivelm} or {in-vehicle communication with human driver}~\citep{deruyttere2022talk2car}. To the best of our knowledge, datasets featuring natural language data for {\textbf{inter-vehicle}} communication are not yet available.

On the other hand, multi-agent {\textbf{``self-play''}} learning in a high-fidelity simulator requires no real-world data and allows for closed-loop learning and evaluation. With recent advances in large language models~(LLMs), there has been a surge of interest in applying LLMs to multi-agent games \citep{meta2022cicero, xu2023werewolf, light2023avalonbench}. However, the synergy between LLMs and multi-agent games remains unexplored in the context of autonomous driving. Existing efforts in autonomous driving mainly focus on leveraging LLMs for decision-making in a \emph{single-agent} setting~\citep{mao2023gptdriver, shao2023lmdrive, ma2023dolphins}.

To enable autonomous agents to learn what to say to cooperate from interactions with each other while still constraining the messages in the natural language space, we propose a novel method, \method, as an initial %\commenta{can we claim "the first attempt"?} 
attempt to use LLMs to help solve the cooperative driving problem in a V2V communication framework. This method optimizes the in-context knowledge of a language model as the message generation {guideline} through a turn-based post-episode discussion{(debriefing)} and leverages LLMs to analyze the dialogue history among neighboring vehicles to generate general driving commands and messages to send. Finally, an atomic controller executes the control according to the updated instructions. To test our method and provide a research test bed for the community, we build a simulation framework containing an array of interesting multi-agent driving scenarios that support communications in natural languages. Our experimental results show an improvement in driving safety and efficiency of our method compared to the methods without communication. 

In summary, this paper makes the following contributions:
\begin{enumerate}[leftmargin=*]
    \item {We present the task of cooperative driving facilitated by vehicle-to-vehicle communication using natural language.}%, aiming to 
    \item We {contribute a multi-agent} simulation framework to realistically model vehicle-to-vehicle communication through natural language, featuring diverse scenarios that capture a range of traffic conditions and interactive challenges.
    \item {We propose a novel method that empowers autonomous vehicles to dynamically generate and integrate natural language messages, facilitating inter-vehicle cooperation and leveraging multi-agent debriefing for improved coordination after interactions.}
    \item We evaluate our methodology within this simulation framework and find that our method is able to generate meaningful messages and improve traffic safety as well as efficiency {compared to alternative approaches}.
\end{enumerate}

==> contents/8_limitation.tex <==
% \newpage
% CoRL requires a page for limitation discussion
\section{Limitations and Future Work} 
\label{sec:limitation}

While our work provides promising initial evidence of the potential of LLM agents and \method{}'s in addressing the \task~problem, it comes with several limitations and opens up rich directions for future research:

\paragraph{Idealized Agent Perception} % In this work, the LLM agents rely on text observations, assuming an idealized perception system. This choice stems from the strong performance of current LLMs and the early-stage development of multi-modal models. However, \simulator~environment supports multi-modal sensory input. Future work should develop agents that integrate multi-sensor perception and reasoning to fully leverage the rich context in realistic observations. 

\paragraph{Communication Challenges}
%We assume that agents intend to communicate truthfully, reliably conveying their intentions and following through on their stated decisions. However, real-world vehicle-to-vehicle communication faces numerous challenges, including time delays that result in outdated information and the risk of adversarial or deceptive messages. Future research should develop methods to handle these challenges, ensuring timely and secure exchanges of information. Techniques such as real-time data verification and robust communication protocols will be critical for enhancing the reliability and safety of vehicle-to-vehicle communication systems.

\paragraph{Training Scalability and Ad Hoc Teamwork}
%While this paper reports on a successful proof-of-concept, the scalability of \method~to learn in diverse traffic scenarios and different environmental conditions has not been exhaustively tested. A limitation of our method is that, although it is sample-efficient, requiring only a few interaction episodes, the analysis must occur immediately after an episode concludes, which hinders scaling up learning. Future work could potentially scale up the training using multi-agent reinforcement learning to finetune the agents while using strong Kullback–Leibler regularization with a foundation model to ensure the agents speak human language during self-play. Additionally, future work should address ad hoc teamwork, where agents adapt to collaborators following different conventions.

\paragraph{Human Interface and Human Evaluation}
%To extend these methods to human-autonomous cooperation, intuitive and user-friendly interfaces (e.g., speech) are essential. Although our research opens up the potential for autonomous cars to cooperate with human drivers, the complexity of effective communication interfaces for humans is substantial. Comprehensive human-centered evaluations using human-friendly interfaces are deferred to future studies.




















%this research opens up several exciting future research areas for further exploration and development. 
%Second, while this paper reports on a successful proof-of-concept, we are interested in scaling the evaluation benchmark and solution to more diverse traffic scenarios and operation conditions resembling real-world V2V communication, e.g., subject to time delays, adversarial attacks, and limited bandwidths. Last, our framework opens up the exciting potential to create a cooperative driving system for mixed-autonomy traffic scenarios. We are interested in realizing this potential, by studying the \task~problem with human-in-the-loop experiments and exploring framework design to enable efficient communication between autonomous vehicles and human drivers.

% \paragraph{Assumptions.}
% In this work, we assume that agents intend to communicate truthfully, accurately conveying their intentions and following through on their stated decisions. 
% While all focal agents are designed to act cooperatively, avoiding deceptive messages or aggressive actions that could disrupt others' driving objectives, we assume that background agents in our framework are not explicitly optimized for cooperation or adversarial behavior. Additionally, we assume that agents communicate in a manner that ensures the syntax and semantics of all messages are human-understandable, such that a human operator could comprehend the exchanged information if analyzing it retrospectively. However, for the purpose of this paper, we do not enforce that the messages are succinct enough for a human driver to understand them in real time while driving.
% Relaxing any (or all) of these assumptions presents interesting directions for future research. 

% \input{Tables/experiment_generalization}

% {
% Although we demonstrate some initial success of \method~in the \task~problem, this research opens up several areas that require further exploration and development.}

% \paragraph{Inference Time.}
% {The response time of large language models (LLMs) can be prohibitive, particularly when rapid decision-making is critical. Currently, it takes several seconds for LLMs to process and respond to prompts, which is too slow for real-time applications. Future efforts could explore model distillation techniques to create smaller, more efficient models that retain the capabilities of their larger counterparts but operate at a faster pace.}











==> contents/acknowledgement.tex <==
\section*{Acknowledgments}
This work has taken place in the Learning Agents Research
Group (LARG) at the Artificial Intelligence Laboratory, The University
of Texas at Austin.  LARG research is supported in part by the
National Science Foundation (FAIN-2019844, NRT-2125858), the Office of
Naval Research (N00014-18-2243), Army Research Office
(W911NF-23-2-0004, W911NF-17-2-0181), DARPA (Cooperative Agreement
HR00112520004 on Ad Hoc Teamwork), Lockheed Martin, and Good Systems,
a research grand challenge at the University of Texas at Austin.  The
views and conclusions contained in this document are those of the
authors alone.  Peter Stone serves as the Executive Director of Sony
AI America and receives financial compensation for this work.  The
terms of this arrangement have been reviewed and approved by the
University of Texas at Austin in accordance with its policy on
objectivity in research.

==> contents/checklist.tex <==
\newpage

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> figure_tex/intro.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.56\textwidth]{Figures/intro.pdf}
    \hfil
    \includegraphics[width=0.375\textwidth]{Figures/intro-1.pdf}
    \caption{\small\textbf{Left:} A red-light violation scenario where there is a car running the red light. \textbf{Right:} An overtake scenario where a truck is broken and stopped on a two-lane two-way road. %\jmh{Text in this figure needs a couple of edits. ex -> "...but since you would be stuck here indefinitely, I will stop for you." otherwise it sounds like something is missing.}
    }
    \label{fig:intro}
\end{figure}

==> figure_tex/qualitative.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/qualitative.pdf}
    \caption{\small Diverse cooperation modes in the Highway Merge negotiation scenario. In this scenario, both vehicles aim to merge quickly as they are in a hurry. \textbf{Top}: The merging vehicle successfully negotiates for the highway vehicles to yield. \textbf{Bottom}: The merging vehicle opts to wait for the highway vehicle to pass before merging. \rev{We refer readers to the demo videos for detailed messages.}} 
    \label{fig:qualitative-highway-merge}
\end{figure}

==> figure_tex/qualitative_cooperative_perception.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{Figures/WeChatf8030954f40f509690b68dee130ae935.jpg}
    \caption{\smallTrajectories in Overtake: Cooperative Perception \jiaxun{TODO: I will make it a trajectory with timestep and corresponding message.}}
    \label{fig:qualitative-cooperative-perception}
\end{figure}

==> figure_tex/qualitative_negotiation.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{Figures/WeChate0de2f85ba0567cd9b62f08c424eba00.jpg}
    \caption{\smallTrajectories in Overtake: Negotiation}
    \label{fig:qualitative-negotiation}
\end{figure}

==> styles/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

